Finding Differentially Covarying Needles in a Temporally Evolving Haystack: A Scan Statistics Perspective

Recent results in coupled or temporal graphical models offer schemes for estimating the relationship structure between features when the data come from related (but distinct) longitudinal sources. A novel application of these ideas is for analyzing group-level differences, i.e., in identifying if trends of estimated objects (e.g., covariance or precision matrices) are different across disparate conditions (e.g., gender or disease). Often, poor effect sizes make detecting the differential signal over the full set of features difficult: for example, dependencies between only a subset of features may manifest differently across groups. In this work, we first give a parametric model for estimating trends in the space of SPD matrices as a function of one or more covariates. We then generalize scan statistics to graph structures, to search over distinct subsets of features (graph partitions) whose temporal dependency structure may show statistically significant group-wise differences. We theoretically analyze the Family Wise Error Rate (FWER) and bounds on Type 1 and Type 2 error. On a cohort of individuals with risk factors for Alzheimer's disease (but otherwise cognitively healthy), we find scientifically interesting group differences where the default analysis, i.e., models estimated on the full graph, do not survive reasonable significance thresholds.

==> prelim-diffgeom.tex <==
%We briefly review some of basic concepts \cite{do1992riemannian} and notations that will be utilized in the remainder of the presentation. For more details, readers can refer to 
{\bf Basic differential geometry notations.} 
%\noindent {\bf Riemannian manifolds.} 
%Before discussion about general regressions models for manifold-valued response variables, let's revisit manifolds.
Let $\Mc$ be a \textit{differentiable (smooth) manifold} in arbitrary dimensions.
%$\Mc$ is a maximal family of \textit{injective} mappings $\varphi_{i}:U_{i}
%\subset \textbf{R}^{n} \rightarrow \Mc$ of open sets $U_{i}$ of
%$\textbf{R}^{n}$ into $\Mc$ such that:
%\begin{inparaenum}[\bfseries (1)]
%\item $\cup_{i} \varphi_i(U_{i}) =\Mc$; 
%\item for any pair $i,j$ with $\varphi_{i} (U_{i}) \cap
%\varphi_{j} (U_{j}) = W \neq \phi$, the sets $\varphi_{i}^{-1}(W)$
%and $\varphi_{j}^{-1}(W)$ are open sets in $\textbf{R}^{n}$ and the
%mappings $\varphi_{j}^{-1} \circ \varphi_{i}$ are
%differentiable, where $\circ$ denotes function composition. 
%\item The family $\{(U_{i},\varphi_{i})\}$ is maximal relative to
%the conditions (1) and (2). 
%\end{inparaenum}
%In other words, 
A differentiable manifold $\Mc$ is a topological
space that is locally similar to Euclidean space and has a globally
defined differential structure. 
%
%A \textit{Riemmannian manifold} is a differentiable manifold $\Mc$ equipped with a smoothly varying inner product $g_p$ in the tangent space ($T_{p}\Mc$) at a point $p$ on the manifold.
%, is a vector space that consists of
%the tangent vectors of {\em all} possible curves passing through $p$. The Tangent bundle of $\Mc$, i.e., $T\Mc$, is the disjoint union of tangent spaces at all points of $\Mc$, 
%$T\Mc = \coprod_{p \in \Mc}T_{p}\Mc$. 
%The tangent bundle is equipped with a natural \textit{projection map} $\pi: T\Mc \rightarrow \Mc$ \cite{lee2012introduction}. 
%
A \textit{Riemannian manifold} is a differentiable manifold $\Mc$ equipped with a smoothly varying inner product.
%The family of inner products on all tangent spaces is known as 
%the \textit{Riemannian metric}, 
%This definition 
%enables us to 
%With Riemannian metrics, we can 
%which defines various geometric notions on curved manifolds such as the length of a curve. 
A \textit{geodesic curve} is a locally shortest path, which is  analogous to straight lines in $\textbf{R}^{p}$ --- such a geodesic 
curve will be the object that defines the trajectory of our covariance matrices in $\SPD$ space. 
Unlike the Euclidean space, note that there may exist multiple geodesic curves between two points on a curved manifold. 
So, the \textit{geodesic distance}
between two points on $\Mc$ is defined as the length of the {\em shortest} geodesic curve connecting two points.
The geodesic distance helps in measuring the error of our trajectory estimation (analogous to a Frobenius or $\ell_2$ norm based loss in the Euclidean setting).
The geodesic curve from $y_i$ to $y_j$  is parameterized by a tangent vector in the tangent space anchored at $y_i$ with an exponential map $\EXP(y_i,\cdot ): T_{y_i}\Mc \rightarrow \Mc$. 
The inverse of the exponential map is the logarithm map, $\LOG(y_i,\cdot):\M \rightarrow T_{y_i}\M$. These two operations move us back and forth between 
the manifold and the tangent space. 
%For completeness, Table \ref{tab:comp} shows corresponding %operations in the Euclidean space and Riemannian manifolds.
%In this paper, we use $\EXP(\cdot, \cdot)$ and $\LOG(\cdot, \cdot)$ for exponential map and its inverse logarithm map for Riemannian manifold. 
Separate from the above notation, matrix exponential (and logarithm) are simply $\exp(\cdot)$ (and $\log(\cdot)$).  
%Lastly, \textit{parallel transport} is a generalized parallel translation on manifolds. 
%Let $\Mc$ be a differentiable manifold with
%an affine connection $\nabla$ and $\mathcal{I}$ be an open interval. 
%Let $g : \mathcal{I} \rightarrow  \Mc$ be a differentiable curve in $\Mc$ and let $V_0$ be a tangent vector in $T_{g(t_0)}\Mc$, where $t_0 \in I$. 
%Then, there exists a unique parallel vector field $V$ along $c$, such that $V (t_0) = V_0$. Here, $V (t)$ is called the parallel transport of $V (t_0)$ along $g$. 
%We denote the parallel transport from $y$ to $y_0$ of $V$ as $\Gamma_{y\rightarrow y'}V$ . Intuitively, parallel transport of $V_0$ along curve $g$ can be interpreted as the parallel translation of $V_0$ on manifolds preserving the angle between $V (t)$ and $g$.
Finally, \textit{parallel transport} is a generalized parallel translation on manifolds. Given a differentiable curve $\gamma : \mathcal{I} \rightarrow  \Mc$, where $\mathcal{I}$ is an open interval, 
the parallel transport of $v_0 \in T_{\gamma(t_0)}\Mc$ along curve $\gamma$ can be interpreted as the parallel translation of $v_0$ on the manifold preserving its length and the angle between $v (t)$ and $\gamma$. 
The parallel transport of $v$ from $y$ to $y'$ is $\Gamma_{y\rightarrow y'}v$.
We include in the appendix additional differential geometry background.
%For , the reader may refer to the supplement (includes a detailed appendix).

%\renewcommand{\arraystretch}{1.5}
%\begin{table}[!b]
%{\footnotesize
%\begin{center}
%    \begin{tabular}{| l | l | l | }
%    \hline
%    Operation & Euclidean & Riemannian  \\  \hline 
%    \footnotesize Subtraction & $\overrightarrow{x_i x_j} = x_j - x_i$ & $\overrightarrow{x_i x_j} = \LOG(x_i,x_j)$ \\ 
%    \footnotesize Addition & $x_i + \overrightarrow{x_j x_k}$ & $\EXP(x_i,\overrightarrow{x_j x_k})$ \\     
%    \footnotesize Distance  & $\| \overrightarrow{x_i x_j} \|$ & $\|\LOG(x_i,x_j) \|_{x_i}$ \\ 
%    Mean  & $\sum_{i=1}^{n} \overrightarrow{\bar{x}x_{i}}=0$ & \footnotesize $\sum_{i=1}^{n} \LOG(\bar{x}, x_i)=0$  \\ 
%    Covariance & \footnotesize$\EE \left [ (x_i - \bar{x})(x_i - \bar{x})^{T} \right ]$&\footnotesize $\EE \left [ \LOG(\bar{x}, x)\LOG(\bar{x}, x)^{T} \right ]$\\ [1ex] \hline 
%  \end{tabular}
%\end{center}
%}
%\caption{\footnotesize Basic operations in Euclidean space and Riemannian manifolds.}
%\label{tab:comp}
%\end{table}

%The interested reader may
%refer to \cite{do1992riemannian} for technical details.

